POCOVID-Net: Automatic Detection of COVID-19 From a New Lung Ultrasound Imaging Dataset (POCUS)

With the rapid development of COVID-19 into a global pandemic, there is an ever more urgent need for cheap, fast and reliable tools that can assist physicians in diagnosing COVID-19. Medical imaging such as CT can take a key role in complementing conventional diagnostic tools from molecular biology, and, using deep learning techniques, several automatic systems were demonstrated promising performances using CT or X-ray data. Here, we advocate a more prominent role of point-of-care ultrasound imaging to guide COVID-19 detection. Ultrasound is non-invasive and ubiquitous in medical facilities around the globe. Our contribution is threefold. First, we gather a lung ultrasound (POCUS) dataset consisting of 1103 images (654 COVID-19, 277 bacterial pneumonia and 172 healthy controls), sampled from 64 videos. This dataset was assembled from various online sources, processed specifically for deep learning models and is intended to serve as a starting point for an open-access initiative. Second, we train a deep convolutional neural network (POCOVID-Net) on this 3-class dataset and achieve an accuracy of 89% and, by a majority vote, a video accuracy of 92% . For detecting COVID-19 in particular, the model performs with a sensitivity of 0.96, a specificity of 0.79 and F1-score of 0.92 in a 5-fold cross validation. Third, we provide an open-access web service (POCOVIDScreen) that is available at: https://pocovidscreen.org. The website deploys the predictive model, allowing to perform predictions on ultrasound lung images. In addition, it grants medical staff the option to (bulk) upload their own screenings in order to contribute to the growing public database of pathological lung ultrasound images. Dataset and code are available from: https://github.com/jannisborn/covid19_pocus_ultrasound. NOTE: This preprint is superseded by our paper in Applied Sciences: https://doi.org/10.3390/app11020672

==> table_data_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Type} & \textbf{Probe} & \textbf{video or photo name}        & \textbf{URL (Video Name)}                                                                                                                                                                                     \\ \hline
video         & convex         & Cov-Atlas+(44).gif                  & http://www.thepocusatlas.com/covid19-1/m2ra6cg22od32eryxmdr7im3qgw714                                                                                                                                         \\ \hline
video         & convex         & Cov-Atlas+(45).gif                  & http://www.thepocusatlas.com/covid19-1/3ytz1el5hly8cq6jigpy0y4irdmy1v                                                                                                                                         \\ \hline
video         & convex         & Cov-Atlas-Day+2.gif                 & http://www.thepocusatlas.com/covid19 (Day2)                                                                                                                                                                   \\ \hline
video         & convex         & Cov-Atlas-Day+4.gif                 & http://www.thepocusatlas.com/covid19 (Day4)                                                                                                                                                                   \\ \hline
video         & convex         & Cov-Butterfly-COVID Lung 2.mp4      & https://www.butterflynetwork.com/covid-19\#lungfindings (Confluent B Lines 2 (23 sec)-deleted from the website)                                                                                               \\ \hline
video         & convex         & Cov-Butterfly-COVID Skip Lesion.mp4 & https://www.butterflynetwork.com/covid-19\#lungfindings (Skip Lesion (44sec) -Category :Other)                                                                                                                \\ \hline
video         & convex         & Cov-clarius.gif                     & https://clarius.com/clinical-utility-and-technique-for-lung-ultrasound-in-covid-19-cases/                                                                                                                     \\ \hline
video         & convex         & Cov-grepmed-blines-pocus-.mp4       & https://www.grepmed.com/images/7415                                                                                                                                                                           \\ \hline
video         & convex         & Cov-grepmed2.mp4                    & https://www.grepmed.com/images/7410                                                                                                                                                                           \\ \hline
video         & convex         & Cov-grepmed3.mp4                    & https://www.grepmed.com/images/7417                                                                                                                                                                           \\ \hline
video         & convex         & Cov-MSU-COVID Lung 2-Blines.mp4     & https://sites.google.com/msu.edu/ (Lung Consolidation)                                                                                                                                                        \\ \hline
video         & convex         & Pneu-Atlas-pneumonia.gif            & http://www.thepocusatlas.com/ (Classic Findings in Pneumonia)                                                                                                                                                 \\ \hline
video         & convex         & pneu-everyday.gif                   & https://everydayultrasound.com/blog/category/Pneumonia                                                                                                                                                        \\ \hline
video         & convex         & pneu-grep-6.gif                     & https://www.grepmed.com/images/5721/airbronchogram-pulmonary-pneumonia-clinical-pocus-lung                                                                                                                    \\ \hline
video         & convex         & Pneu-grep-pneumonia1.mp4            & https://www.grepmed.com/images/6903                                                                                                                                                                           \\ \hline
video         & convex         & Pneu-grep-pneumonia2.mp4            & https://www.grepmed.com/images/6876                                                                                                                                                                           \\ \hline
video         & convex         & Pneu-grep-pneumonia4.mp4            & https://www.grepmed.com/images/6431                                                                                                                                                                           \\ \hline
video         & convex         & pneu-radiopaeda.mp4                 & https://radiopaedia.org/cases/pneumonia-ultrasound-1                                                                                                                                                          \\ \hline
video         & convex         & Reg-Atlas-lungcurtain.gif           & http://www.thepocusatlas.com/ (Lung Curtain)                                                                                                                                                                  \\ \hline
video         & convex         & Reg-Atlas.gif                       & http://www.thepocusatlas.com/ (Improve Lung Sliding Visualization)                                                                                                                                            \\ \hline
video         & convex         & Reg-bcpocus.gif                     & https://www.bcpocus.ca/organscans/pneumonia/                                                                                                                                                                  \\ \hline
video         & convex         & Reg-Butterfly.mp4                   & https://www.butterflynetwork.com/covid-19\#lungfindings (Normal Lung Example 1)                                                                                                                               \\ \hline
video         & convex         & Reg-NormalLungs.mp4                 & https://radiopaedia.org/cases/normal-anterior-lung-ultrasound-1                                                                                                                                               \\ \hline
video         & convex         & Reg-Youtube.mp4                     & https://www.youtube.com/watch?v=VzgX9ihnmec                                                                                                                                                                   \\ \hline
video         & convex         & Cov-Atlas-+(43).gif                 & http://www.thepocusatlas.com/covid19-1/ru6w5sgjyu1zn21jraypm2pfm0h6uf                                                                                                                                         \\ \hline
video         & convex         & Cov-Atlas-Day+1.gif                 & http://www.thepocusatlas.com/covid19 (Day1)                                                                                                                                                                   \\ \hline
video         & convex         & Cov-Atlas-Day+3.gif                 & http://www.thepocusatlas.com/covid19 (Day3)                                                                                                                                                                   \\ \hline
video         & convex         & Cov-Butterfly-COVID Lung 1.mp4      & https://www.butterflynetwork.com/covid-19\#lungfindings (Confluent B Lines (27 sec))                                                                                                                          \\ \hline
video         & convex         & Cov-MSU-SkipLesions.mp4             & https://sites.google.com/msu.edu/ (Skip Lesions)                                                                                                                                                              \\ \hline
video         & convex         & Pneu-Atlas-pneumonia-AirBronch.gif  & http://www.thepocusatlas.com/ (Dynamic Air Bronchograms in Pneumonia)                                                                                                                                         \\ \hline
video         & convex         & pneu-grep-7.gif                     & https://www.grepmed.com/images/1304/airbronchograms-pneumonia-sonostuff-clinical-effusion-pocus-lung                                                                                                          \\ \hline
video         & convex         & Pneu-grep-pneumonia3.mp4            & https://www.grepmed.com/images/6439                                                                                                                                                                           \\ \hline
video         & convex         & Reg-Atlas-alines.gif                & http://www.thepocusatlas.com/ (A-Lines-Normal Lung)                                                                                                                                                           \\ \hline
video         & convex         & Reg-Grep-Alines.mp4                 & https://www.grepmed.com/images/7408                                                                                                                                                                           \\ \hline
video         & convex         & Reg-Grep-Normal.gif                 & https://www.grepmed.com/images/5325                                                                                                                                                                           \\ \hline
video         & convex         & Reg-nephropocus.mp4                 & https://nephropocus.com/2019/06/03/lung-ultrasound-a-line-and-b-lines/\#jp-carousel-642                                                                                                                       \\ \hline
photo         & convex         & Cov-B\_ConvexProb\_score1.jpg       & Publication: Proposal for international standardization of the use of lung ultrasound for COVID‐19 patients \cite{soldati2020proposal} \\ \hline
photo         & convex         & Cov-C\_Convex\_Prob\_score2.jpg     & Publication: Proposal for international standardization of the use of lung ultrasound for COVID‐19 patients \cite{soldati2020proposal} \\ \hline
photo         & convex         & Cov-D\_Convex\_Prob\_score3.jpg     & Publication: Proposal for international standardization of the use of lung ultrasound for COVID‐19 patients \cite{soldati2020proposal} \\ \hline
photo         & convex         & Cov-C\_ConvexProb\_score3.jpg       & Publication: Proposal for international standardization of the use of lung ultrasound for COVID‐19 patients \cite{soldati2020proposal} \\ \hline
\end{tabular}%
}
\caption{List of sources for all files in the the dataset}
\label{data_source_table}
\end{table*}
